Real-time Neural Radiance Caching for Path Tracing

We present a real-time neural radiance caching method for path-traced global illumination. Our system is designed to handle fully dynamic scenes, and makes no assumptions about the lighting, geometry, and materials. The data-driven nature of our approach sidesteps many difficulties of caching algorithms, such as locating, interpolating, and updating cache points. Since pretraining neural networks to handle novel, dynamic scenes is a formidable generalization challenge, we do away with pretraining and instead achieve generalization via adaptation, i.e. we opt for training the radiance cache while rendering. We employ self-training to provide low-noise training targets and simulate infinite-bounce transport by merely iterating few-bounce training updates. The updates and cache queries incur a mild overhead -- about 2.6ms on full HD resolution -- thanks to a streaming implementation of the neural network that fully exploits modern hardware. We demonstrate significant noise reduction at the cost of little induced bias, and report state-of-the-art, real-time performance on a number of challenging scenarios.

==> __latexindent_temp.tex <==

\section{Variance of CV Estimator}
\label{sec:variance-derivation}

We are interested in deriving the variance of the following estimator:
\begin{align}
    \MC{F} = \CV(\CVParams) + \frac{f(X,Z)}{\PdfMC(X,Z)}  - \frac{\cv(X;\cvParams)}{\PdfMC(X)} \,.
    \label{eq:mc-integrator-with-z-appendix}
\end{align}
To simplify the derivation, we subtract the constant $\CV(\CVParams)$ from both sides and proceed with the definition of variance:
\begin{align}
    \Variance\left[\MC{F} - \CV(\CVParams)\right] &= \Expectation\left[ \left({\MC{F} - \CV(\CVParams)}\right)^2 \right] - {\Expectation\left[ \MC{F} - \CV(\CVParams) \right]}^2
    \,.
    \label{eq:mc-variance-derivation-appendix}
\end{align}
Since $\Variance[X + c] = \Variance[X]$, the left-hand side simplifies to $\Variance\left[\MC{F}\right]$.
The expectation of the square can be expressed as the following double integral:
\begin{align}
    \Expectation\left[ \left({\MC{F} \!-\! \CV(\CVParams)}\right)^2 \right]
    \!&=
    \Expectation\left[ \left(
        \frac{f(X,Z)}{\PdfMC(X,Z)}  - \frac{\cv(X;\cvParams)}{\PdfMC(X)}
    \right)^2 \right] \nonumber\\
    &=\!\! \int_\Domain \! \int_\DomainZ \!\! \left( \frac{f(x,z)}{\PdfMC(x,z)} - \frac{\cv(x;\cvParams)}{\PdfMC(x)}\right)^2
     \PdfMC(x,z) \Diff{z}\!\Diff{x}
    \nonumber \\
    &=\!\! \int_\Domain \! \int_\DomainZ \!\! \left( \frac{f(x,z)}{\PdfMC(x)\PdfMC(z|x)} - \frac{\cv(x;\cvParams)}{\PdfMC(x)}\right)^2
     \!\PdfMC(x)\PdfMC(z|x) \Diff{z}\!\Diff{x}
    \nonumber \\
    &=\!\! \int_\Domain \! \int_\DomainZ \!\! \left( \frac{f(x,z)}{\PdfMC(z|x)} - \cv(x;\cvParams)\right)^2\frac{\PdfMC(z|x)}{\PdfMC(x)} \Diff{z}\!\Diff{x}
\label{eq:mc-expectation-of-square-appedix}
\end{align}
The squared expectation (second term in \autoref{eq:mc-variance-derivation-appendix}) simplifies to $\left(\Expectation\left[\MC{F}\right] - \CV(\CVParams) \right)^2 = \left(F - \CV(\CVParams) \right)^2$.
Putting all the terms together yields \autoref{eq:mc-variance-with-tail}.



\section{Variance Gradients}
\label{sec:variance-gradient-derivation}
We derive gradients for two estimators: 1) an estimator with a parametric CV and a \emph{fixed} sampler for estimating the difference integral, and 2) an estimator with parametric CV and a parametric, \emph{trainable} sampler (such as those proposed by \citet{mueller2019nis}).

\subsection{Trainable CV and Fixed Sampler}
For ease of notation, we split the variance function into two terms, $A$ and $B$:
\begin{align}
    \Variance\left[\MC{F}\right]
    &= \underbrace{\!\int_\Domain \!\int_\DomainZ \! \left( \frac{f(x,z)}{\PdfMC(z|x)} - \cv(x;\cvParams)\right)^2\frac{\PdfMC(z|x)}{\PdfMC(x)} \Diff{z}\!\Diff{x}}_{A}
    - \underbrace{(F - \CV(\CVParams))^2}_{B}.
\label{eq:mc-variance-with-tail-appendix}
\end{align}
The variance gradient $\nabla_{\cvParams} \Variance\left[\MC{F}\right] = \nabla_{\cvParams} A - \nabla_{\cvParams} B$ consists of the following:
\begin{align}
\nabla_{\cvParams}A
&= \nabla_{\cvParams}\!\int_\Domain \!\int_\DomainZ \! \left( \frac{f(x,z)}{\PdfMC(z|x)} - \cv(x;\cvParams)\right)^2\frac{\PdfMC(z|x)}{\PdfMC(x)} \Diff{z}\!\Diff{x}
\nonumber\\
&= \!\int_\Domain \!\int_\DomainZ \!\nabla_{\cvParams} \left( \frac{f(x,z)}{\PdfMC(z|x)} - \cv(x;\cvParams)\right)^2\frac{\PdfMC(z|x)}{\PdfMC(x)} \Diff{z}\!\Diff{x}
\nonumber\\
&= -2 \int_\Domain
\frac{ \int_\DomainZ f(x,z) - \cv(x;\cvParams) \PdfMC(z|x)  \Diff{z} }{\PdfMC(x)}
\nabla_{\cvParams} \cv(x;\cvParams)
\Diff{x}
\nonumber\\
&= -2 \int_\Domain
\frac{f(x) - \cv(x;\cvParams) }{\PdfMC(x)}
\nabla_{\cvParams} \cv(x;\cvParams)
\Diff{x}\,,
\\
\nonumber\\
\nabla_{\cvParams}B
&= \nabla_{\CVParams} \left(F - \CV(\CVParams)\right)^2
\nonumber\\
&= -2\, \left(F - \CV(\CVParams)\right) \,\nabla_{\CVParams} \CV(\CVParams)\,.
\label{eq:mc-variance-with-tail-appendix}
\end{align}
Putting the terms together:
\begin{align}
\nabla_{\cvParams} \Variance\left[\MC{F}\right] =
&-2 \int_\Domain
\frac{f(x) - \cv(x;\cvParams) }{\PdfMC(x)}
\nabla_{\cvParams} \cv(x;\cvParams)
\Diff{x}\\
&+2\, \left(F - \CV(\CVParams)\right) \,\nabla_{\CVParams} \CV(\CVParams)\,.
\end{align}

Since the gradient cannot be evaluated in closed form (due to the presence of integral $F$, which is unknown, and likely also because of the difference integral), we can estimate the two integrals using the following one-sample estimator:
\begin{align}
    \MC{\nabla_{\cvParams} \Variance\left[\MC{F}\right]} =
    &-2
    \frac{\MC{f(x)} - \cv(x;\cvParams) }{\PdfMC(x) \PdfVarEst(x)}
    \nabla_{\cvParams} \cv(x;\cvParams)
    \\
    &+2\, \left(\frac{\MC{f(x)}}{\PdfVarEst(x)} - \CV(\CVParams)\right) \,\nabla_{\CVParams} \CV(\CVParams)\,.
\end{align}
The above estimator is unbiased as long as $\MC{f(x)}$ is unbiased: the other terms merely scale and offset $\MC{f(x)}$ preserving the zero-mean distribution of the stochastic error.



\subsection{Trainable CV and Trainable Sampler}
We now consider the case of a parametric, optimizable probability density $\PdfMC(x;\pdfParams)$.


\begin{align}
    \nabla_{\Params}A
    &= \nabla_{\Params}\!\int_\Domain \!\int_\DomainZ \! \left( \frac{f(x,z)}{\PdfMC(z|x)} - \cv(x;\cvParams)\right)^2\frac{\PdfMC(z|x)}{\PdfMC(x;\pdfParams)} \Diff{z}\!\Diff{x}
    \nonumber\\
    &=
    \int_\Domain \int_\DomainZ
    - \frac{\PdfMC(z|x) \left(\frac{f(x,z)}{\PdfMC(z|x)} - \cv(x;\cvParams)\right)
    \left(
        \left(\frac{f(x,z)}{\PdfMC(z|x)} - \cv(x;\cvParams) \right)  \nabla_{\pdfParams}\PdfMC(x;\pdfParams)
        +
        2 \PdfMC(x;\pdfParams) \nabla_{\cvParams} \cv(x, \cvParams)
    \right)
    }{ \PdfMC(x;\pdfParams)^2 }
    \label{eq:mc-variance-with-tail-appendix}
    \end{align}


\newpage
\onecolumn
I'm curious how you derived the gradient in the case of NCV+NIS.
Let's just focus on the following term of variance:
\begin{align}
    \int_\Domain  \frac{ (f - \cv(\cvParams))^2}{\PdfMC(\pdfParams)} \Diff{x}
\end{align}
Denoting $\Params = \cvParams \cup \pdfParams$, we can derive the gradient using the product rule:
\begin{align}
    \nabla_{\Params}  \int_\Domain  \frac{ (f - \cv(\cvParams))^2}{\PdfMC(\pdfParams)} \Diff{x}
    &=
    \int_\Domain \nabla_{\Params}  \left( (f - \cv(\cvParams))^2 \cdot \frac{1}{\PdfMC(\pdfParams)} \right)  \Diff{x}
    \\
    &= \int_\Domain \left(-2 (f - \cv(\cvParams)) \nabla_{\cvParams} \cv(\cvParams)   \frac{1}{\PdfMC(\pdfParams)} \right)
    +
    \left(\right)
    \\
\end{align}
